On Turn-Regular Orthogonal Representations

An interesting class of orthogonal representations consists of the so-called turn-regular ones, i.e., those that do not contain any pair of reflex corners that "point to each other" inside a face. For such a representation H it is possible to compute in linear time a minimum-area drawing, i.e., a drawing of minimum area over all possible assignments of vertex and bend coordinates of H. In contrast, finding a minimum-area drawing of H is NP-hard if H is non-turn-regular. This scenario naturally motivates the study of which graphs admit turn-regular orthogonal representations. In this paper we identify notable classes of biconnected planar graphs that always admit such representations, which can be computed in linear time. We also describe a linear-time testing algorithm for trees and provide a polynomial-time algorithm that tests whether a biconnected plane graph with "small" faces has a turn-regular orthogonal representation without bends.

==> app-small-faces.tex <==
In this section, we give the detailed proof of Theorem~\ref{th:small-faces} in Section~\ref{sec:rect}.

%\begin{theorem}\label{th:small-faces}
%  Let $G$ be a biconnected plane graph with faces of degree at most~8. There exists a polynomial-time algorithm that decides whether $G$ admits an embedding-preserving rectilinear turn-regular representation and that computes such a representation in the positive case. 
%\end{theorem}
\thsmallfaces*
\begin{proof}
We describe a testing algorithm based on a constrained version of Tamassia's flow network $N(G)$, which models the space of orthogonal representations of $G$ within its given planar embedding~\cite{DBLP:journals/siamcomp/Tamassia87}.
We briefly recall how $N(G)$ is defined and then we describe how to modify it for our testing algorithm.
Let $V$, $E$, and $F$ be the set of vertices, edges, and faces of $G$, respectively. $N(G)$ is a directed multigraph. It has a \emph{vertex-node} $\nu_v$ for each vertex $v \in V$ and a \emph{face-node} $\nu_f$ for each face $f \in F$.
Also, $N(G)$ has two types of edges: $(i)$ for each vertex $v$ of a face $f$, there is a directed edge $(\nu_v,\nu_f)$ with capacity~3; $(ii)$ for each edge $e \in E$, denoted by $f$ and $g$ the two faces incident to $e$, there is a directed edge $(\nu_f,\nu_g)$ and a directed edge $(\nu_g,\nu_f)$, both with infinite capacity.

A feasible flow on $N(G)$ corresponds to an orthogonal representation of $G$. Each unit of flow on an edge of $N(G)$ represents an angle of $90^\circ$ (at a vertex or at a bend) in the corresponding orthogonal representation. More precisely, a flow value $k \in \{1,2,3\}$ on an edge $(\nu_v,\nu_f)$ represents an angle of $90 \cdot k$ degrees at $v$ in $f$ (since $G$ is biconnected, there is no angle larger than $270^\circ$ at a vertex); a flow value $k \geq 0$ on an edge $(\nu_f,\nu_g)$ represents $k$ bends on the edge of $G$ associated with $(\nu_f,\nu_g)$, and all these bends form an angle of $90^\circ$ inside $f$. 
Since the sum of the angles at a vertex $v \in V$ is $360^\circ$, each vertex-node $\nu_v$ supplies 4 units of flow in $N(G)$. At the same time, each face-node $\nu_f$ in $N(G)$ demands an amount of flow equal to $c_f = (2\deg(f)-4)$ if $f$ is internal and to $c_f = (2\deg(f)+4)$ if $f$ is external. The value $c_f$ represents the \emph{capacity of} $f$.  It is proved in~\cite{DBLP:journals/siamcomp/Tamassia87} that the total flow supplied by the vertex-nodes equals the total flow demanded by the face-nodes; if a face-node $\nu_f$ cannot consume all the flow supplied by its adjacent vertex-nodes (because its capacity $c_f$ is smaller), it can send the exceeding flow to an adjacent face-node $\nu_g$, through an edge $(\nu_f,\nu_g)$, thus originating bends.  

Our algorithm has to test the existence of an orthogonal representation $H$ such that: (a) $H$ has no bend; (b) $H$ is turn-regular. To this aim, we suitably modify $N(G)$ so that the possible feasible flows only model the set of orthogonal representations that verify Properties~(a) and~(b). To enforce Property~(a), we just remove from $N(G)$ the edges between face-nodes. On the opposite, to enforce Property~(b), we enhance $N(G)$ with additional nodes and edges. Consider first an internal face $f$ of $G$. By hypothesis $\deg(f) \leq 8$. It is immediate to see that if $\deg(f) \leq 7$ then $f$ cannot have a pair of kitty corners under the assumption that each edge has no bend. If $\deg(f)=8$, a pair $\{u,v\}$ of kitty corners necessarily requires three vertices along the boundary of $f$ going from $u$ to $v$ (and hence also from $v$ to $u$); see Fig.~\ref{fig:small-faces-1}. Therefore, for such a face $f$, we locally modify $N(G)$ around $\nu_f$ as shown in Fig.~\ref{fig:small-faces-2}. Namely, for each potential pair $\{u,v\}$ of kitty corners, we introduce an intermediate node $\nu_{uv}$; the original edges $(\nu_u,\nu_f)$ and $(\nu_v,\nu_f)$ are replaced by the edges $(\nu_u,\nu_{uv})$ and $(\nu_v,\nu_{uv})$, respectively (each still having capacity 3); finally, an edge $(\nu_{uv},\nu_f)$ with capacity $5$ is inserted, which avoids that $u$ and $v$ form a reflex corner inside $f$ at the same time.  
For the external face $f$, and under the assumption that all the edges are straight, it can be easily seen that a pair of kitty corners is possible only if the face has degree at least 10. Since we are assuming that $\deg(f) \leq 8$, we do not need to apply any local modification to $N(G)$ for the external face.

Hence, a rectilinear turn-regular representation of $G$ corresponds to a feasible flow in the modified version of $N(G)$. Since $N(G)$ can be easily transformed into a sparse unit capacity network, this problem can be solved in $O(n^{1.5})$ time by applying a maximum flow algorithm (the value of the maximum flow must be equal to $4|V|$)~\cite{DBLP:books/daglib/0069809}.
\end{proof}


